WiPLoc: Perpetual Indoor Localization with RF Wireless Power Transfer

Indoor localization is a cornerstone of mobile services. Until now most of the research effort has focused on achieving sub-meter localization accuracy because many mobile applications depend on precise localization measurements. In some scenarios, however, it is required to trade location accuracy for system maintainability. For example, in large-scale deployments of indoor networks, such as item-monitoring in smart buildings, attaining room-level localization accuracy may be sufficient, but replacing the batteries of the devices used for localization could lead to high operational costs. As indoor localization systems grow in popularity it will be important to provide them with full energy autonomy. To tackle this problem we propose WiPLoc: an indoor localization system aimed at operating perpetually without batteries. Our contributions are twofold. First, we propose a novel localization method that exploits capture effect and orthogonal codes to operate at energy levels that are low enough to operate within the energy budget provided by long-range wireless power transmission. Second, we implement WiPLoc using off-the-shelf components and test it extensively in a laboratory environment. Our test results show that with WiPLoc one wireless charger per (16 m$^{\text{2}}$) room can enable perpetual lifetime operation of mobile objects requiring localization with an average accuracy of almost 90%.

==> title_IEEE.tex <==
\title{WiPLoc: Perpetual Indoor Localization with RF
Wireless Power Transfer}


% author names and affiliations
% use a multiple column layout for up to three different
% affiliations
\author{\IEEEauthorblockN{Michael Shell}
\IEEEauthorblockA{School of Electrical and\\Computer Engineering\\
Georgia Institute of Technology\\
Atlanta, Georgia 30332--0250\\
Email: http://www.michaelshell.org/contact.html}
\and
\IEEEauthorblockN{Homer Simpson}
\IEEEauthorblockA{Twentieth Century Fox\\
Springfield, USA\\
Email: homer@thesimpsons.com}
\and
\IEEEauthorblockN{James Kirk\\ and Montgomery Scott}
\IEEEauthorblockA{Starfleet Academy\\
San Francisco, California 96678--2391\\
Telephone: (800) 555--1212\\
Fax: (888) 555--1212}}

% conference papers do not typically use \thanks and this command
% is locked out in conference mode. If really needed, such as for
% the acknowledgment of grants, issue a \IEEEoverridecommandlockouts
% after \documentclass

% for over three affiliations, or if they all won't fit within the width
% of the page, use this alternative format:
% 
%\author{\IEEEauthorblockN{Michael Shell\IEEEauthorrefmark{1},
%Homer Simpson\IEEEauthorrefmark{2},
%James Kirk\IEEEauthorrefmark{3}, 
%Montgomery Scott\IEEEauthorrefmark{3} and
%Eldon Tyrell\IEEEauthorrefmark{4}}
%\IEEEauthorblockA{\IEEEauthorrefmark{1}School of Electrical and Computer Engineering\\
%Georgia Institute of Technology,
%Atlanta, Georgia 30332--0250\\ Email: see http://www.michaelshell.org/contact.html}
%\IEEEauthorblockA{\IEEEauthorrefmark{2}Twentieth Century Fox, Springfield, USA\\
%Email: homer@thesimpsons.com}
%\IEEEauthorblockA{\IEEEauthorrefmark{3}Starfleet Academy, San Francisco, California 96678-2391\\
%Telephone: (800) 555--1212, Fax: (888) 555--1212}
%\IEEEauthorblockA{\IEEEauthorrefmark{4}Tyrell Inc., 123 Replicant Street, Los Angeles, California 90210--4321}}




% use for special paper notices
%\IEEEspecialpapernotice{(Invited Paper)}




% make the title area
\maketitle
